Benefits and Harms of Large Language Models in Digital Mental Health

The past decade has been transformative for mental health research and practice. The ability to harness large repositories of data, whether from electronic health records (EHR), mobile devices, or social media, has revealed a potential for valuable insights into patient experiences, promising early, proactive interventions, as well as personalized treatment plans. Recent developments in generative artificial intelligence, particularly large language models (LLMs), show promise in leading digital mental health to uncharted territory. Patients are arriving at doctors' appointments with information sourced from chatbots, state-of-the-art LLMs are being incorporated in medical software and EHR systems, and chatbots from an ever-increasing number of startups promise to serve as AI companions, friends, and partners. This article presents contemporary perspectives on the opportunities and risks posed by LLMs in the design, development, and implementation of digital mental health tools. We adopt an ecological framework and draw on the affordances offered by LLMs to discuss four application areas -- care-seeking behaviors from individuals in need of care, community care provision, institutional and medical care provision, and larger care ecologies at the societal level. We engage in a thoughtful consideration of whether and how LLM-based technologies could or should be employed for enhancing mental health. The benefits and harms our article surfaces could serve to help shape future research, advocacy, and regulatory efforts focused on creating more responsible, user-friendly, equitable, and secure LLM-based tools for mental health treatment and intervention.

==> 00packages.tex <==
\usepackage{tikz}
\usepackage{capt-of}
\usepackage{subcaption, balance}
\usepackage{balance,bm}
\usepackage{enumitem}
% \usepackage{natbib}

\captionsetup{compatibility=false}
\usepackage [english]{babel}
\usepackage{url}
\usepackage [autostyle, english = american]{csquotes}
\definecolor{linkColor}{RGB}{6,125,233}
\definecolor{green}{rgb}{0.0, 0.65, 0.31}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\definecolor{grey}{HTML}{969696}
\definecolor{violet}{HTML}{756bb1}
\definecolor{dgrey}{HTML}{01665e}
\definecolor{lgrey}{HTML}{5ab4ac}
\definecolor{dgreen}{HTML}{005a32}
\definecolor{purple}{HTML}{ae017e}
%pt, bp, dd, mm, cm, ex, em, pc, in
\def\greybar#1{{\color{grey}\rule{#1pc}{6pt}}}
\def\dgreybar#1{{\color{dgrey}\rule{#1pc}{6pt}}}
\def\lgreybar#1{{\color{lgrey}\rule{#1pc}{6pt}}}
% \definecolor{editCol}{rgb}{0.0, 0.3, 0.5}
\definecolor{editCol}{rgb}{0.1, 0.1, 0.8}
% \definecolor{editCol}{HTML}{000000}
\definecolor{maskCol}{HTML}{c51b7d}
\definecolor{lrColor}{HTML}{8856a7}
\definecolor{trColor}{HTML}{d01c8b}
\definecolor{ctColor}{HTML}{4dac26}
\definecolor{brickred}{HTML}{f03b20}
\definecolor{improveCol}{HTML}{253494}
\definecolor{worsenCol}{HTML}{d7191c}
\definecolor{DarkBlue}{HTML}{00008B}
\definecolor{dolive}{HTML}{308014}

\usepackage{mathtools}

\usepackage{tcolorbox}

\usepackage{amsmath, amssymb}
\usepackage{array}
\usepackage{xcolor}
\usepackage{arydshln}
\setlength\dashlinedash{0.2pt}
\setlength\dashlinegap{1.5pt}
\setlength\arrayrulewidth{0.3pt}
\usepackage{siunitx}

\usepackage{fancyhdr}   % custom header/footer
\fancypagestyle{firststyle}{%
   \fancyfoot{}
   \fancyhead[RO,LE]{\small\sffamily{\thepage}}
}

\def\impbar#1{%%
  {\color{improveCol}\rule{#19mm}{5pt}}
  }
\def\worbar#1{%%
  {\color{worsenCol}\rule{#19mm}{5pt}}
  }
\def\trbar#1{%%
  {\color{trColor}\rule{#19mm}{5pt}}
  }
\def\mybar#1{%%
  {\color{bleudefrance}\rule{#19mm}{5pt}}
  }
\def\nubarGreen#1{%%
  {\color{neutralGreen}\rule{#19mm}{5pt}}
  }
 \def\nubar#1{%%
  {\color{neutralCol}\rule{#19mm}{5pt}}
  }
\def\BfBar#1{%%
  {\color{BfTrColor}\rule{#19mm}{5pt}}
  } 
  \def\AfBar#1{%%
  {\color{AfTrColor}\rule{#19mm}{5pt}}
  }
\newcommand*{\textlabel}[2]{%
  \edef\@currentlabel{#1}% Set target label
  \phantomsection% Correct hyper reference link
  #1\label{#2}% Print and store label
}


 
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\colorlet{tableheadcolor}{gray!25} % Table header colour = 25% gray
\newcommand{\headcol}{\rowcolor{tableheadcolor}} %
\colorlet{tablerowcolor}{gray!15} % Table row separator colour = 
\colorlet{tablerowcolor2}{gray!25} % Table row separator colour = 10% gray
\newcommand{\rowcol}{\rowcolor{tablerowcolor}} %
\newcommand{\rowcollight}{\rowcolor{tablerowcolor2}} %
% \newcommand{\rowcollight}{\rowcolor{NewBlue}} %

\newcommand{\Pon}{$P_1$}
\newcommand{\Ptw}{$P_2$}
\newcommand{\Pth}{{$P_3$}}
\newcommand{\Con}{$C_1$}
\newcommand{\Ctw}{$C_2$}
\newcommand{\Cth}{{$C_3$}}

\newif{\ifhidecomments}
 \hidecommentsfalse 
%\hidecommentstrue
\ifhidecomments
    \newcommand{\koustuv}[1]{}
    \newcommand{\vedant}[1]{}
    \newcommand{\gregory}[1]{}
    \newcommand{\munmun}[1]{}
\else
    \newcommand{\vedant}[1]{\textbf{\small\sffamily{\textcolor{purple}{[#1 -- Vedant]}}}}
    \newcommand{\koustuv}[1]{\textbf{\small\sffamily{\textcolor{DarkBlue}{[#1 -- Koustuv]}}}}
    \newcommand{\gregory}[1]{\textbf{\small\sffamily{\textcolor{dolive}{[#1 -- Gregory]}}}}
    \newcommand{\munmun}[1]{\textbf{\small\sffamily{\textcolor{brickred}{[#1 -- Munmun]}}}}
  \fi
% \newcommand{\edit}[1]{{\textcolor{editCol}{#1}}}
\newcommand{\edit}[1]{{#1}}
\newcommand{\mask}[1]{{\textcolor{maskCol}{#1}}}

\def\nuLRbar#1{%%
  {\color{lrColor}\rule{#10mm}{4pt}}
  }
\newcommand{\Bf}{\textsl{Before}}
\newcommand{\Af}{\textsl{After}}
\newcommand{\Tr}{\textsl{Treatment}}
\newcommand{\Cs}{\textsl{Case}}
\newcommand{\Ct}{\textsl{Control}}
% \newcommand{\M}{\textsl{Scenario M}}
% \newcommand{\Sn}{\textsl{Scenario 1}}
% \newcommand{\Snn}{\textsl{Scenario 2}}
% \newcommand{\Snnn}{\textsl{Scenario 3}}
\newcommand{\M}{$S_M$}
\newcommand{\Sn}{$S_1$}
\newcommand{\Snn}{$S_2$}
\newcommand{\Snnn}{$S_3$}
\newcommand{\RTE}{\textsl{RTE}}
\newcommand{\ITE}{\textsl{ITE}}
\newcommand{\ea}{\textit{et al.}}
% \newcommand{\imp}[1]{{\textcolor{improveCol}{\it#1}}}
% \newcommand{\wor}[1]{{\textcolor{worsenCol}{\it#1}}}
\newcommand{\imp}[1]{{\textcolor{improveCol}{\it#1}}}
\newcommand{\wor}[1]{{\textcolor{worsenCol}{\it#1}}}

\newcommand{\del}{\textsl{C\textsubscript{1}}}
\newcommand{\gar}{\textsl{C\textsubscript{2}}}
\newcommand{\und}{\textsl{C\textsubscript{3}}}
\newcommand{\CL}{\textsl{CampusLife}}
\newcommand{\BD}{\textsl{Bipolar}}
\newcommand{\BPD}{\textsl{Borderline}}
\newcommand{\CT}{\textsl{Control}}
\newcommand{\MV}{\textsl{MI}}
\newcommand{\HMV}{\textsl{High MI}}
\newcommand{\LMV}{\textsl{Low MI}}
% \newcommand{\oc}{\texttt{}{OC}}
\newcommand{\oc}{\textsl{OC}}


\newcommand{\pro}{\textit{Pros}}
\newcommand{\con}{\textit{Cons}}
\newcommand{\mo}{\textit{Model 1}}
\newcommand{\moo}{\textit{Model 2}}

\renewcommand{\textrightarrow}{$\rightarrow$}
\renewcommand{\textleftarrow}{$\leftarrow$}

\newcommand{\cdib}{$\mathbf{CDI}$}
% \newcommand{\somra}{$\mathnormal{LibRA}$}
\newcommand{\cdi}{$\mathtt{CDI}$}

% \newcommand{\somra}{\mathcal{SoMRA}}
\newcommand{\somrab}{$\mathbf{LibRA}$}
% \newcommand{\somra}{$\mathnormal{LibRA}$}
\newcommand{\somra}{$\mathtt{LibRA}$}




% \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\colorlet{tableheadcolor}{gray!25} % Table header colour = 25% gray
% \newcommand{\headcol}{\rowcolor{tableheadcolor}} %
\colorlet{tablerowcolor}{gray!5} % Table row separator colour = 10% gray
% \newcommand{\rowcol}{\rowcolor{tablerowcolor}} %

\definecolor{neutralCol}{HTML}{dd1c77}
\definecolor{neutralGreen}{HTML}{31a354}
\definecolor{NewBlue}{HTML}{1879ba}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}  
\definecolor{AfTrColor}{HTML}{0868ac}  
\definecolor{BfTrColor}{HTML}{a8ddb5}  

\definecolor{AfCtColor}{HTML}{b10026}  
\definecolor{BfCtColor}{HTML}{fd8d3c}

\graphicspath{ {figures/} }

\def\plaintitle{Drug Effects}
\def\plainauthor{First Author, Second Author, Third Author,
  Fourth Author, Fifth Author, Sixth Author}
\def\emptyauthor{}
\def\plainkeywords{mental health, social media, Twitter, psychiatric medication use, causal inference, precision psychiatry, drug effects}

